DPOAD: Differentially Private Outsourcing of Anomaly Detection through Iterative Sensitivity Learning

Outsourcing anomaly detection to third-parties can allow data owners to overcome resource constraints (e.g., in lightweight IoT devices), facilitate collaborative analysis (e.g., under distributed or multi-party scenarios), and benefit from lower costs and specialized expertise (e.g., of Managed Security Service Providers). Despite such benefits, a data owner may feel reluctant to outsource anomaly detection without sufficient privacy protection. To that end, most existing privacy solutions would face a novel challenge, i.e., preserving privacy usually requires the difference between data entries to be eliminated or reduced, whereas anomaly detection critically depends on that difference. Such a conflict is recently resolved under a local analysis setting with trusted analysts (where no outsourcing is involved) through moving the focus of differential privacy (DP) guarantee from "all" to only "benign" entries. In this paper, we observe that such an approach is not directly applicable to the outsourcing setting, because data owners do not know which entries are "benign" prior to outsourcing, and hence cannot selectively apply DP on data entries. Therefore, we propose a novel iterative solution for the data owner to gradually "disentangle" the anomalous entries from the benign ones such that the third-party analyst can produce accurate anomaly results with sufficient DP guarantee. We design and implement our Differentially Private Outsourcing of Anomaly Detection (DPOAD) framework, and demonstrate its benefits over baseline Laplace and PainFree mechanisms through experiments with real data from different application domains.

==> backup.tex <==
 \begin{figure*}[!tbh]
	\centering
% 	\subfigure[Round]{
% 		\includegraphics[angle=0, width=0.3\linewidth]{1_rr_TP}
% 		\label{fig:1_rr_TP} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Recall]{
		\includegraphics[angle=0, width=0.23\linewidth]{1_rr_Re}
		\label{fig:1_rr_Re} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Precision]{
		\includegraphics[angle=0, width=0.23\linewidth]{1_rr_Pre}
		\label{fig:1_rr_Pre}}
		%\hspace{-0.15in}
% 	\caption{Evaluation of three mechanisms with parking dataset for different accuracy metrics}
% 	\label{fig:1_rr_data}
% \end{figure*}
% \begin{figure*}[!tbh]
% 	\centering
% 	\subfigure[Round]{
% 		\includegraphics[angle=0, width=0.3\linewidth]{2_rr_TP}
% 		\label{fig:2_rr_TP} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Recall]{
		\includegraphics[angle=0, width=0.23\linewidth]{2_rr_Re}
		\label{fig:2_rr_Re} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Precision]{
		\includegraphics[angle=0, width=0.23\linewidth]{2_rr_Pre}
		\label{fig:2_rr_Pre}}
		%\hspace{-0.15in}
	\caption{Rounds v.s. Recall and Precision in parking dataset (a) and (b) and electric consumption (c) and (d)}
	\label{fig:2_rr_data}
\end{figure*}

\begin{figure*}[!tbh]
	\centering
% 	\subfigure[Round]{
% 		\includegraphics[angle=0, width=0.3\linewidth]{4_rr_TP}
% 		\label{fig:4_rr_TP} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Recall]{
		\includegraphics[angle=0, width=0.23\linewidth]{4_rr_Re}
		\label{fig:4_rr_Re}}
		%\hspace{-0.15in}
	\subfigure[Round v.s. Precision]{
		\includegraphics[angle=0, width=0.23\linewidth]{4_rr_Pre}
		\label{fig:4_rr_Pre}}
		%\hspace{-0.15in}
% 	\caption{Evaluation of three mechanisms with credit card dataset for different accuracy metrics}
% 	\label{fig:4_rr_data}
% \end{figure*}
% \begin{figure*}[!tbh]
% 	\centering
% 	\subfigure[Round]{
% 		\includegraphics[angle=0, width=0.3\linewidth]{5_rr_TP}
% 		\label{fig:5_rr_TP} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Recall]{
		\includegraphics[angle=0, width=0.23\linewidth]{5_rr_Re}
		\label{fig:5_gam_Re} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Precision]{
		\includegraphics[angle=0, width=0.23\linewidth]{5_rr_Pre}
		\label{fig:5_rr_Pre}}
		%\hspace{-0.15in}
	\caption{Round v.s. Recall and Precision in credit card dataset (a) and (b) and KDD dataset (c) and (d)}
	\label{fig:5_rr_data}
\end{figure*}

\begin{figure*}[!tbh]
	\centering
% 	\subfigure[Round]{
% 		\includegraphics[angle=0, width=0.3\linewidth]{S_rr_TP}
% 		\label{fig:S_rr_TP} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Recall]{
		\includegraphics[angle=0, width=0.23\linewidth]{S_rr_Re}
		\label{fig:S_rr_Re} }
		%\hspace{-0.15in}
	\subfigure[Round v.s. Precision]{
		\includegraphics[angle=0,width=0.23\linewidth]{S_rr_Pre}
		\label{fig:S_rr_Pre}}
		%\hspace{-0.15in}
% 	\caption{Evaluation of three mechanisms with MERL dataset for different accuracy metrics}
% 	\label{fig:S_rr_data}
% \end{figure*}
%  %round exp end%
% \begin{figure*}[!tbh]
% 	\centering
% 	\subfigure[Round]{
% 		\includegraphics[angle=0, width=0.3\linewidth]{Den_rr_TP}
% 		\label{fig:Den_T_TP} }
		%\hspace{-0.15in}
	\subfigure[Round]{
		\includegraphics[angle=0, width=0.23\linewidth]{Den_rr_Re}
		\label{fig:Den_rr_Re} }
		%\hspace{-0.15in}
	\subfigure[Round]{
		\includegraphics[angle=0, width=0.23\linewidth]{Den_rr_Pre}
		\label{fig:Den_rr_Pre}}
		%\hspace{-0.15in}
	\caption{Round v.s. Recall and Precision in MERL dataset (a) and (b) and traffic monitoring dataset (c) and (d)}
	\label{fig:Den_rr_data}
\end{figure*}


\begin{table*}[!h]
 \centering\small
 \caption{Round v.s. Recall and Precision}
 Parking Datase\\
 \vspace{0.05in}
 %\renewcommand\arraystretch{1.2}
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
  &Round &1&2&3&4\\
  \hline
  %\toprule
 %\multirow{2}{*}{Round $\#$} &
 %\multicolumn{2}{c|}{\texttt{1}} & 
 %\multicolumn{2}{c|}{\texttt{2}}  & 
 %\multicolumn{2}{c|}{\texttt{3}} & 
 %\multicolumn{2}{c|}{\texttt{4}} \\
%\cline{2-3}\cline{4-5}\cline{6-7}\cline{8-9}
% &Precision &  Recall & Precision &  Recall  &   Precision &  Recall& Precision &  Recall\\
 % \hline
  %\toprule
 % \cline{5-6}\cline{7-8}\cline{9-10}\cline{11-12}
%  & &  Recall &   Recall  &  Recall &  Recall  & Recall\\
  %\midrule
\multirow{2}{*}{Laplace} & Precision & & & &	\\
\cline{2-6}
& Recall & & & &	\\
\hline
\multirow{2}{*}{Painfree} & Precision & & & &	\\
\cline{2-6}
& Recall & & & &	\\
\hline
\multirow{2}{*}{DPOAD} & Precision & & & &	\\
\cline{2-6}
& Recall & & & &	\\
\hline
%Painfree & 	98.1\% &  	98.1\% &  98.1\% &  99.0\%&	98.1\% &	98.1\% &	98.1\% &	98.7\% \\
%\hline
%DPOAD &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
%\hline
\end{tabular}

 Parking Datase\\
 \vspace{0.05in}
 %\renewcommand\arraystretch{1.2}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  &Round &1&2&3&4&&1&2&3&4\\
  \hline
  %\toprule
 %\multirow{2}{*}{Round $\#$} &
 %\multicolumn{2}{c|}{\texttt{1}} & 
 %\multicolumn{2}{c|}{\texttt{2}}  & 
 %\multicolumn{2}{c|}{\texttt{3}} & 
 %\multicolumn{2}{c|}{\texttt{4}} \\
%\cline{2-3}\cline{4-5}\cline{6-7}\cline{8-9}
% &Precision &  Recall & Precision &  Recall  &   Precision &  Recall& Precision &  Recall\\
 % \hline
  %\toprule
 % \cline{5-6}\cline{7-8}\cline{9-10}\cline{11-12}
%  & &  Recall &   Recall  &  Recall &  Recall  & Recall\\
  %\midrule
\multirow{2}{*}{Laplace} & Precision & & & & &&&& &	\\
\cline{2-11}
& Recall & & & &&&&&&	\\
\hline
\multirow{2}{*}{Painfree} & Precision & & & &&&&&&	\\
\cline{2-11}
& Recall & & & &&&&&&	\\
\hline
\multirow{2}{*}{DPOAD} & Precision & & & &&&&&&	\\
\cline{2-11}
& Recall & & & &&&&&&	\\
\hline
%Painfree & 	98.1\% &  	98.1\% &  98.1\% &  99.0\%&	98.1\% &	98.1\% &	98.1\% &	98.7\% \\
%\hline
%DPOAD &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
%\hline
\end{tabular}

Electric Consumption Dataset\\
 \vspace{0.05in}
    \begin{tabular}{|c|cc|cc|cc|cc|}
  \hline
  %\toprule
 \multirow{2}{*}{Round $\#$} &
 \multicolumn{2}{c|}{\texttt{1}} & 
 \multicolumn{2}{c|}{\texttt{2}}  & 
 \multicolumn{2}{c|}{\texttt{3}} & 
 \multicolumn{2}{c|}{\texttt{4}} \\
\cline{2-3}\cline{4-5}\cline{6-7}\cline{8-9}
 &Precision &  Recall & Precision &  Recall  &   Precision &  Recall& Precision &  Recall\\
  \hline
  %\toprule
 % \cline{5-6}\cline{7-8}\cline{9-10}\cline{11-12}
%  & &  Recall &   Recall  &  Recall &  Recall  & Recall\\
  %\midrule
Laplace &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
Painfree & 	98.1\% &  	98.1\% &  98.1\% &  99.0\%&	98.1\% &	98.1\% &	98.1\% &	98.7\% \\
\hline
DPOAD &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
\end{tabular}
 
 \vspace{0.05in} 
 Credit Card Dataset\\
 \vspace{0.05in}
    \begin{tabular}{|c|cc|cc|cc|cc|}
  \hline
  %\toprule
 \multirow{2}{*}{Round $\#$} &
 \multicolumn{2}{c|}{\texttt{1}} & 
 \multicolumn{2}{c|}{\texttt{2}}  & 
 \multicolumn{2}{c|}{\texttt{3}} & 
 \multicolumn{2}{c|}{\texttt{4}} \\
\cline{2-3}\cline{4-5}\cline{6-7}\cline{8-9}
 &Precision &  Recall & Precision &  Recall  &   Precision &  Recall& Precision &  Recall\\
  \hline
  %\toprule
 % \cline{5-6}\cline{7-8}\cline{9-10}\cline{11-12}
%  & &  Recall &   Recall  &  Recall &  Recall  & Recall\\
  %\midrule
Laplace &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
Painfree & 	98.1\% &  	98.1\% &  98.1\% &  99.0\%&	98.1\% &	98.1\% &	98.1\% &	98.7\% \\
\hline
DPOAD &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
\end{tabular}
 
 \vspace{0.05in} 
KDD Dataset\\
 \vspace{0.05in}
   \begin{tabular}{|c|cc|cc|cc|cc|}
  \hline
  %\toprule
 \multirow{2}{*}{Round $\#$} &
 \multicolumn{2}{c|}{\texttt{1}} & 
 \multicolumn{2}{c|}{\texttt{2}}  & 
 \multicolumn{2}{c|}{\texttt{3}} & 
 \multicolumn{2}{c|}{\texttt{4}} \\
\cline{2-3}\cline{4-5}\cline{6-7}\cline{8-9}
 &Precision &  Recall & Precision &  Recall  &   Precision &  Recall& Precision &  Recall\\
  \hline
  %\toprule
 % \cline{5-6}\cline{7-8}\cline{9-10}\cline{11-12}
%  & &  Recall &   Recall  &  Recall &  Recall  & Recall\\
  %\midrule
Laplace &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
Painfree & 	98.1\% &  	98.1\% &  98.1\% &  99.0\%&	98.1\% &	98.1\% &	98.1\% &	98.7\% \\
\hline
DPOAD &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
\end{tabular}
 
 \vspace{0.05in}    
 MERL Dataset\\
 \vspace{0.05in}
    \begin{tabular}{|c|cc|cc|cc|cc|}
  \hline
  %\toprule
 \multirow{2}{*}{Round $\#$} &
 \multicolumn{2}{c|}{\texttt{1}} & 
 \multicolumn{2}{c|}{\texttt{2}}  & 
 \multicolumn{2}{c|}{\texttt{3}} & 
 \multicolumn{2}{c|}{\texttt{4}} \\
\cline{2-3}\cline{4-5}\cline{6-7}\cline{8-9}
 &Precision &  Recall & Precision &  Recall  &   Precision &  Recall& Precision &  Recall\\
  \hline
  %\toprule
 % \cline{5-6}\cline{7-8}\cline{9-10}\cline{11-12}
%  & &  Recall &   Recall  &  Recall &  Recall  & Recall\\
  %\midrule
Laplace &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
Painfree & 	98.1\% &  	98.1\% &  98.1\% &  99.0\%&	98.1\% &	98.1\% &	98.1\% &	98.7\% \\
\hline
DPOAD &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
\end{tabular}
 
  \vspace{0.05in}    
 MERL Dataset\\
 \vspace{0.05in}
   \begin{tabular}{|c|cc|cc|cc|cc|}
  \hline
  %\toprule
 \multirow{2}{*}{Round $\#$} &
 \multicolumn{2}{c|}{\texttt{1}} & 
 \multicolumn{2}{c|}{\texttt{2}}  & 
 \multicolumn{2}{c|}{\texttt{3}} & 
 \multicolumn{2}{c|}{\texttt{4}} \\
\cline{2-3}\cline{4-5}\cline{6-7}\cline{8-9}
 &Precision &  Recall & Precision &  Recall  &   Precision &  Recall& Precision &  Recall\\
  \hline
  %\toprule
 % \cline{5-6}\cline{7-8}\cline{9-10}\cline{11-12}
%  & &  Recall &   Recall  &  Recall &  Recall  & Recall\\
  %\midrule
Laplace &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
Painfree & 	98.1\% &  	98.1\% &  98.1\% &  99.0\%&	98.1\% &	98.1\% &	98.1\% &	98.7\% \\
\hline
DPOAD &	98.1\% &	98.1\% &	98.1\% &	98.7\% &	98.1\% &	98.1\% &	98.1\% &	98.7\%\\
\hline
\end{tabular}
 \end{table*}
 
 


==> intro1.tex <==
\section{Introduction}
	\label{intro4}


  





While differential privacy provably obscures the presence
or absence of individual records in a dataset, it has a major limitation: the analysis results
are randomized w.r.t the maximum possible difference one single individual can make in the final result, namely the \textit{sensitivity} of the analysis. Defining sensitivity in context of network anomalies detection is not straightforward as one may contribute numerous number of records to the dataset which results in a very high value of sensitivity, stronger randomization mechanism and hence less useful analysis results. This has led the community to consider a record-level differentially private solution~\cite{McSherry:2010:DNT:1851275.1851199} (sensitivity is fixed to be one) which results in a weak level of protection taking the multi-accessibility of nature of network traces (in comparison to relational databases) into account.  We show that this approach is effective (utility preserving) and justifiable in IDS that leverage hypothesis testing in their solutions. In particular, such solutions are entitled to enforce a data pre-analysis to approximate the conditional probability distribution of different anomalies.






As the owners of large-scale network data, today's ISPs and
enterprises usually face a dilemma. %As security monitoring and
% analytics grow more sophisticated, there is an increasing need for
% those organizations to outsource such tasks together with necessary
% network data to third-party analysts, e.g., Managed Security Service
% Providers (MSSPs)~\cite{10.1007/11600930_96}.
% Moreover, 
A number of network security and monitoring problems
can substantially benefit if a group of involved organizations
aggregates private data to jointly perform a
computation. For example, IDS alert correlation, e.g.,
with DOMINO~\cite{Yegneswaran04globalintrusion}, requires the joint analysis of private
alerts. Similarly, aggregation of private data is useful
for alert signature extraction~\cite{Parekh:2006:PPC:1162666.1162667}, collaborative anomaly
detection~\cite{Boggs2011CrossDomainCA}, multi-domain traffic engineering~\cite{Machiraju2004VerifyingGI}, detecting
traffic discrimination~\cite{Tariq:2009:DNN:1658939.1658972}, and collecting network
performance statistics~\cite{10.1007/978-3-540-24668-8_17}.
On the other hand, those
organizations are typically reluctant to share their network trace
data with third parties, and even less willing to publish them, mainly
due to privacy concerns over sensitive information contained in such
data. For example, important network configuration information, such
as potential bottlenecks of the network, may be inferred from network
traces and subsequently exploited by adversaries to increase the
impact of a denial of service attack~\cite{6195626}.

There have been several studies on collaborative anomaly detection, where a number of participants want to build a global model from their local records,
while none of the participants are willing to disclose their private data. 
Most existing work relies on the use of \textit{Secure Multiparty Computation} (SMC) to
generate the global model for anomaly detection~\cite{6063441,5497205,Burkhart:2010:RNT:1672308.1672310}. While this approach can
achieve high levels of protocol privacy and accuracy, SMC incurs a high communication and computational overhead and in some scenarios is subjected to infeasibility of being implemented due to lack of capability, e.g., IoT systems and smart home.
 Moreover, unauthorized parties participated in a SMC-based collaborative protocol may infer some sensitive data about one of the participants through exploiting the computed result. \hl{For instance, a certain port number which is flagged by the distributed IDS can communicate the fact that the other participant is experiencing a vulnerability on that specific port.} Moreover, SMC based methods require the simultaneous coordination of all participants during the entire training process, which
limits the number of participants. Thus, an open research challenge is how to
improve scalability while achieving high levels of accuracy and privacy.
To address this challenge, several efforts have devoted to propose a convincing privacy-preserving scheme. Unfortunately, these efforts are entitled to serious deficiencies including ad hoc definition of privacy and weak problem statement. In particular, M. Erfani et al.~\cite{10.1007/978-3-319-06608-0_48} present a new definition of privacy called \textit{Random Multiparty Perturbation} (RMP) which is not an accredited definition of privacy leading to the fact that one cannot assure the RMP output will be protected against different side channel attacks. On  the other hand, differential privacy has
been widely recognized as the
state-of-the-art~\cite{Dwork08differentialprivacy:,10.1007/11681878_14} privacy preserving scheme. By requiring the presence of any individual's data in the input to only marginally affect the
distribution over the output, differential privacy provides strong protection against adversaries in with arbitrary background
knowledge about the individuals.  

 While differential privacy provably obscures the presence
or absence of individual records in a dataset, in some applications, differential privacy is in contradiction with the analysis, e.g., in finding anomalies where generating indistinguishable query results (DP) contradicts the anomaly detection procedure.

  Mcssherry et al. ~\cite{McSherry:2009:PIQ:1559845.1559850} was first that proposed a differentially private network trace analysis was done by benchmarking with the Privacy Integrated
Queries (PINQ). Unfortunately, applying PINQ directly to the network traces through the queries pertains a serious privacy violation. Specifically, the strength of the randomization in a differentially private mechanism, to answer a query, is specified by a characteristics of the query and the dataset, called the \textit{sensitivity} of the query, which is defined as the maximum value of a difference one individual can make in the output of the query. In the context of network trace analysis, one individual may contribute several records to the dataset resulting in a larger than one sensitivity, whereas the Privacy Integrated
Queries (PINQ) assumes a sensitivity equal to one (similar to counting queries). 

\subsection{Motivation}
Our key observation is that, most existing works in privacy preserving network trace analysis are unable to find the realistic relation between \DP and the semantic of network data, mainly due to the problematic definition of the sensitivity for this type of datasets. Specifically, if the sensitivity is considered as the maximum value of a deviation, one individual can make, the randomization will fully destroy the usefulness of the data (one IP address may have so many activities). On the other hand, smaller value for sensitivity may violate the privacy of individuals drastically.

To address the aforementioned issue, this paper proposes a novel recursive approach called \textit{No \DP for Anomalies} taking into account the fact that most of anomalies are subjected to a certain detection threshold when being identified, and those thresholds are defined relatively higher than what a normal-behavior can conduct. The key idea here is for the data owner to recursively identify and exclude the set of identified anomalies from his/her dataset with the goal of estimating a reasonably lower sensitivity and hence smaller noise injection. For this purpose, we first assume that the sensitivity of each analysis to be a random variable which with a higher probability returns a smaller value according to the external knowledge available for the analysis.
As shown in Figure~\ref{fig:2}, this probability distribution is then updated in different recursion when the results of the collaborative detection are returned to data owners. Moreover, we formulate our problem in a setting when a sequential hypothesis testing IDS is deployed. This choice of IDS is because (1) sequential hypothesis testing generates reliable alarms~\cite{1301325,5714699} (2) the probabilistic nature of these IDS, and especially, the sound formulation of the detection errors can be incorporated in estimating the probability distribution of the sensitivity.   


% Intuitively, by neglecting the privacy of the data of one individual (IP address) which is flagged as an anomaly behavior, we  (1) If the anomaly is a true anomaly then we are neglecting the privacy of a malicious user. (2) If the anomaly is a false positive, then we violate the privacy which will be corrected in next iterations 
\begin{figure}[tb] \centering
	\includegraphics[width=1.1\linewidth, viewport=160 60 830 420,clip]{Overview.pdf}
\caption{An overview of the DP-IDS}
\label{fig:2}
\end{figure}
%  \begin{figure*}[ht]
% \includegraphics[width=1\linewidth]{ov.pdf}
% \centering
% \caption{An overview of the R$^2$DP approach. Comparison between traditional Laplace mechanism and a sample result of R$^2$DP for $\epsilon=0.9$ is depicted.}
% \label{figoverview}
% \end{figure*}
\begin{figure*}[tb] \centering
	\includegraphics[width=0.85\linewidth, viewport=160 60 1300 720,clip]{Over.pdf}
\caption{An overview of the DP-IDS}
\label{fig:3}
\end{figure*}
\subsection{Contributions}
Specifically, DP-IDS makes the following technical contributions to
improve the usability of differentially private collaborative IDS in practice:
\begin{enumerate}
    \item DP-IDS proposes a realistic model of differentially private network trace analysis by assuming a randomized sensitivity value.
    \item DP-IDS sacrifices the privacy of the anomalies to preserve the privacy of data with normal behavior while boosting the accuracy of the analysis by iteratively refining the the sensitivity definition using the computed IDS results.

\item The general concept of sensitivity reinement in DP-IDS can be adapted to improve a
  variety of other applications related to differential privacy when we deal with a multi-access (in contrast to single access) datasets e.g.,
  URL data~\cite{6951353} and when each data owner is an IoT device like smart frig, smart light, etc., which has not enough computational resource to perform the analysis locally, or to run a SMC protocol to perform it jointly with other devices. 
    %  ~\cite{Hardt:2010:GDP:1806689.1806786},~\cite{7944526,Barak:2007:PAC:1265530.1265569, Mohammady:2018:PBP:3243734.3243809,7039716,Qardaji:2013:UHM:2556549.2556576, 1fac2e61af8547b39fac891a12435f45,6228069,LiHRMM10, XiaoWG10,Yuan:2015:OBL:2799368.2699501, Li:2014:DWA:2732269.2732271} 

\item We address various challenges raised by the complex nature of
  the two-folded randomization used in DP-IDS, and we give an optimization problem to maximize the utility of our solution .

\item We formally benchmark DP-IDS under the Laplace mechanism for four different network analyses, e.g., port-scanning~\cite{1301325},worm finger-printing~\cite{Cheetancheri:2006:DHW:1162666.1162668}, distributed denial of service~\cite{4359399}.


%   discuss other mechanisms in Sections~\ref{sec:R$^2$DP as a Patch to
%     Existing Work} and Appendix~\ref{sec:Gauss} due to space limitations.


% both
%   machine learning and social network applications, by benchmarking
%   with the Privacy Integrated Queries (PINQ) \cite{McSherry09}. The
%   experimental results have demonstrated that R$^2$DP can
%   significantly increase the utility of these data analyses (e.g.,
%   more than 230\% of the utility of the baseline in PINQ).
\end{enumerate}
% The rest of the paper is organized as follows. Section~\ref{sec:model}
% presents an overview of our R$^2$DP framework together with some
% background information on differential privacy. Section~\ref{sec4} formally
% studies the \DP guarantee of the framework. Section~\ref{sec5}
% analyzes the utility of the framework. Section~\ref{sec:R$^2$DP as a
%   Patch to Existing Work} provides further discussions. Section~\ref{exp:sec} presents the experimental results. 
% Section~\ref{relat} reviews the related work.  Finally,
% Section~\ref{sec:conclusion} concludes the paper.

==> outline.tex <==
% 1. Motivate the main idea of using analysis result to improve the privacy utility trade-off by saying:
% in some application differential privacy is in contradiction with the analysis, i.e., in finding anomalies, the fact that we make the query result indistinguishable contradicts the anomaly detection procedure. 
% Question: is there any way to address such contradiction? yes, it is to apply a recursive solution 1. normal DP and next,  recursively use the analysis result to only make non-anomalies distinguishable. other solutions like SMC is not feasible in scenarios like iot and smart homes as they cannot use smc results by themseleves. moreover, the problem with the no privacy for anomalies to be not fair considering the inaccuracies or some oulier are legitimate, no more exists for these applications. 

% as soon as we go with recursive, some problem will show up: extra overhead and composition which they should be at least naively addressed.
% discussion at least 5 including iot and nfv and then network stuff...
% exp could be done on anomaly detection for networks
% optimization is optional


Convincing scenario:

 

A number of network security and monitoring problems can substantially benefit if a group of involved organizations aggregates private data to jointly perform a computation.

However, by exerting these approaches some private data typically have to be revealed. Most existing work relies on the use of \textit{Secure Multiparty Computation} (SMC) to

generate the global model for anomaly detection~\cite{6063441,5497205,Burkhart:2010:RNT:1672308.1672310}. While this approach can

achieve high levels of protocol privacy and accuracy, SMC incurs a high communication and computational overhead and in some scenarios is subjected to in feasibility of being implemented due to lack of capability, e.g., IoT systems and smart home.

 

In this Paper, we consider the potential for Intrusion Detection Systems (IDS) while providing the strong guarantees of "differential privacy". While differential privacy provably obscures the presence

or absence of individual records in a dataset, in some applications, the very concept of indistinguishability ensured by differential privacy is in contradiction with the analysis, e.g., in finding anomalies where generating indistinguishable query results (DP) contradicts the anomaly detection procedure.

 

Question: is there any way to address such contradiction? yes, it is to apply a recursive solution.

 

However, as soon as we go with a recursive solution, two main problems are needed to be tackled: 1. Extra overhead and 2. Composition leakage due to the multi-round solution (they should be at least naively addressed).

 

 

Other comments:

1.       Disclosing privacy of outliers in general is not justifiable. Therefore, in our model section, we say that we only consider those scenarios that our solution is applicable, e.g., IoT systems where privacy of outliers can be compromised.

2.       Optimization of the protocol can be done to some extent but is the biggest deal.

3.       We may present at least 5 different applications, including IoT and NFV , to justify the applicability of our solution whereas the experiments could be done on anomaly detection attacks.

 

 

Main idea for the recursive solution:

 

The usefulness (utility definition) of a DP mechanism depends on the sensitivity and the privacy guarantee, e.g., the output of a Laplace mechanism is (gamma, exp(-epsilon*gamma/sensitivity))-useful. Suppose a two-round recursive solution:

Round 1: Naïve eps1-DP solution using Laplace and with maximum sensitivity definition (a potentially anomaly activity is also considered as privacy-sensitive data).

Round 2: Import the collaborative results to see if the sensitivity can be degraded. This part can be done probabilistically based on the quality of the anomaly detection results which has been discussed in literature, e.g., an anomality factor in range of [0,100] was proposed, we then use this probabilistic evaluation to degrade sensitivity. Now suppose alpha is the attenuation rate of the sensitivity due to that process, and eps2 is the DP of second round.

Then the usefulness and the privacy guarantee of the overall (2-round) process will be

 

exp(-eps2*gamma/(alpha*sensitivity))-useful & eps1+eps2-DP

 

 

respectively. Now, we can find a straightforward relation between alpha and eps1 and eps2 so that our solution improves the baseline=>    (1/alpa-1)> eps1/ eps2

 

Of course, this requires more discussion on ow to optimally implement the solution (overhead which is the number of round, rrelation between epsilons and finally relation between attenuation rate and quality of detection)
